Simple vs Optimal Mechanisms in Auctions with Convex Payments

We investigate approximately optimal mechanisms in settings where bidders' utility functions are non-linear; specifically, convex, with respect to payments (such settings arise, for instance, in procurement auctions for energy). We provide constant factor approximation guarantees for mechanisms that are independent of bidders' private information (i.e., prior-free), and for mechanisms that rely to an increasing extent on that information (i.e., detail free). We also describe experiments, which show that for randomly drawn monotone hazard rate distributions, our mechanisms achieve at least 80\% of the optimal revenue, on average. Both our theoretical and experimental results show that in the convex payment setting, it is desirable to allocate across multiple bidders, rather than only to bidders with the highest (virtual) value, as in the traditional quasi-linear utility setting.

==> acknowledgments.tex <==

\section{Acknowledgments}



==> app_monopoly.tex <==


\subsection{Proof of Theorem~\ref{thm:apxRatioMonopReserveDgeTwo}}

\begin{proof}
By Lemma~\ref{lem:dhangwatnotai},
\begin{align}
e \eta (1 - F(\eta)) \ge \mu
.\end{align}
%
So by Corollary~\ref{cor:optUbByPseudoSurplusFordtwo},
$OPT$ is upper-bounded by
\begin{align}
OPT
\le 
\numbidders^{(d-1)/d} \left(e \eta (1 - F(\eta))\right)^{1/d}
.\end{align}
%
By Lemma~\ref{lem:reserveQuantileApx}, $APX$ is lower-bounded by
\begin{align}
APX
\ge 
\numbidders
\left(
\frac{\eta}%
{1 + (\numbidders - 1) (1 - F(\eta))}
\right)^{1/d}
(1 - F(\eta))
.\end{align}
%
Using our bounds for $APX$ and $OPT$, we can now describe the performance of the mechanism:
\begin{align}
\frac{APX}{OPT}
&\ge
\numbidders
\left(
\frac{\eta}%
{1 + (\numbidders - 1) (1 - F(\eta))}
\right)^{1/d}
(1 - F(\eta))
\frac{1}{\numbidders^{(d-1)/d} \left(e \eta (1 - F(\eta))\right)^{1/d}}
\\
&=
\numbidders^{1/d}
\left(
\frac{1}%
{1 + (\numbidders - 1) (1 - F(\eta))}
\right)^{1/d}
(1 - F(\eta))^{(d-1)/d}
\frac{1}{e^{1/d}}
\\
&=
\left(
\frac{1}{e}
\frac{\numbidders (1 - F(\eta))^{d-1}}{1 + (\numbidders - 1) (1 - F(\eta))}
\right)^{1/d}
.\end{align}
\end{proof}

\begin{comment}
We note that the guarantees given by 
Theorem~\ref{thm:apxRatioMedianDgeTwo} and
Theorem~\ref{thm:apxRatioMonopReserveDgeTwo}
do not coincide when $\eta = \kappa$.
Notice that 
Theorem~\ref{thm:apxRatioMedianDgeTwo} uses 
$OPT
\le
\numbidders^{(d-1)/d} (e \kappa)^{1/d}$,
while
Theorem~\ref{thm:apxRatioMonopReserveDgeTwo}
invokes
$OPT
\le 
\numbidders^{(d-1)/d} \left(e \eta (1 - F(\eta))\right)^{1/d}$.
Beginning with Equation~\eqref{eq:apxRatioMonopReserveDgeTwo},
since $F(\eta) = F(\kappa)$, we have:
\begin{align}
\frac{APX}{OPT}
&\ge
\left(
\frac{1}{e}
\frac{\numbidders (1 - F(\kappa))^{d-1}}{1 + (\numbidders - 1) (1 - F(\kappa))}
\right)^{1/d}
\\
&=
\left(
\frac{1}{e}
\frac{\numbidders (1/2)^{d-1}}{1 + (\numbidders - 1) (1/2)}
\right)^{1/d}
\\
&=
\left(
\frac{1}{e}
\frac{2 \numbidders (1/2)^{d-1}}{2 + (\numbidders - 1)}
\right)^{1/d}
\\
&=
\frac{1}{2}
\left(
\frac{1}{e}
\frac{4 \numbidders}{\numbidders + 1}
\right)^{1/d}
.\end{align}
%
This tells us that for large $\numbidders$, the approximation ratio is 
$\frac{1}{2}
\left( \frac{4}{e} \right)^{1/d}$.
When $d = 2$, it is approximately $0.6$.
When $d$ is large, it approaches $\frac{1}{2}$.
However, by using a different bound on $OPT$ 
in Theorem~\ref{thm:apxRatioMedianDgeTwo},
we derive a better bound when $\eta = \kappa$.

\begin{theorem}
\label{thm:apxRatioMedianMean}
The approximation ratio of the mechanism with median reserve price $\kappa$
in a symmetric environment, when, $\forall i \in \bidders$, 
$\costfun[i] = \payment[i]^d$, 
where $d \ge 2$, 
and valuations are drawn from a regular distribution,
is:
\begin{align}
\label{eq:apxRatioMedianMean}
\frac{APX}{OPT}
&\ge
\frac{1}{2}
\left( \frac{2 \numbidders \kappa}{ \mu (\numbidders + 1)} \right)^{1/d}
.\end{align}
\end{theorem}

\begin{proof}
Lemma~\ref{lem:reserveQuantileApx} tells us that when $\hat{q} = \frac{1}{2}$,
\begin{align}
APX
&\ge
\frac{\numbidders}{2}
\left(
\frac{2 \kappa}
{\numbidders + 1}
\right)^{1/d}
,\end{align}
%
and by Corollary~\ref{cor:optUbByPseudoSurplusFordtwo},
\begin{align}
OPT
&\le
\numbidders^{(d-1)/d} \mu^{1/d}
.\end{align}
%
Combining the two results, we have
%
\begin{align}
\frac{APX}{OPT}
&\ge
\frac{\numbidders}{2}\left(
\frac{2 \kappa}{\numbidders + 1}\right)^{1/d} 
\frac{1}{\numbidders^{(d-1)/d} \mu^{1/d}}
\\
&=
\frac{1}{2}
\left( \frac{2 \numbidders \kappa}{ \mu (\numbidders + 1)} \right)^{1/d}
.\end{align}
\end{proof}

Consider a setting where $\eta = \kappa = \mu$, as in the case of a uniform distribution.
Then, for large $\numbidders$, the approximation ratio is $\frac{2^{-d}}{2}$.
When $d = 2$, it is approximately $0.7$, and for large $d$, the ratio approaches $\frac{1}{2}$.
\end{comment}


==> reserve_price.tex <==

\section{Mechanisms with a Reserve Price}

We now describe mechanisms where a reserve price is set based on
the bidders' distributions of valuations.
These mechanisms allocate uniformly across the $Z$ winners
and charge ex-post truthful payments.
We begin with a mechanism that sets the reserve price to 
the median of the distribution, $\kappa$,
and compare it to a mechanism that sets the reserve price to
the monopoly reserve, $\eta = v (q^*)$.

\begin{lemma}
\label{lem:reserveQuantileApx}
Let $\val(\hat{q})$ be the reserve price
in a symmetric environment with regular distributions, 
when, $\forall i \in \bidders$, 
$\costfun[i] = \payment[i]^d$, 
where $d \ge 1$.
%
Let $APX$ be the expected revenue of a mechanism that allocates
uniformly across all $Z$ winners  
and charges ex-post truthful payments $(\val(\hat{q}) / Z)^{1/d}$.
Then:
\begin{align}
APX
&\ge
\numbidders
\left(
\frac{\val(\hat{q})}%
{1 + (\numbidders - 1) \hat{q}}
\right)^{1/d}
\hat{q}
.\end{align}
\end{lemma}

\begin{proof}
The expected revenue the mechanism with reserve price $\val(\hat{q})$ is
\begin{align}
APX
&=
\Exp_{\valvec \sim F}
\left[
\sum_{i = 1}^{\numbidders}
\left(
\frac{\val(\hat{q}) \mathbbm{1}_{\val[i] \ge \val(\hat{q})}}%
{\sum_{j = 1}^{\numbidders} \mathbbm{1}_{\val[j] \ge \val(\hat{q})}}
\right)^{1/d}
\right]
.\end{align}
%
The probability that $\val[i] \ge \val(\hat{q})$ is 
$1 - F(\val(\hat{q})) = \hat{q}$, 
and if there exists a winner, the denominator is at least one,
so
\begin{align}
APX
&=
\Exp_{\valvec \sim F}
\left[
\sum_{i = 1}^{\numbidders}
\left(
\frac{\val(\hat{q})}%
{1 + \sum_{j = 1}^{\numbidders-2} \mathbbm{1}_{\val[j] \ge \val(\hat{q})}}
\right)^{1/d}
\right] \hat{q}
\\
&=
\sum_{i = 1}^{\numbidders}
\Exp_{\valvec \sim F}
\left[
\left(
\frac{1}%
{1 + \sum_{j = 1}^{\numbidders - 1} \mathbbm{1}_{\val[j] \ge \val(\hat{q})}}
\right)^{1/d}
\right] 
\val(\hat{q})^{1/d}
\hat{q}
.\end{align}
%
The function 
$h(x) = 1/(1+x)^{1/d}$
is convex for $d \ge 1$.
By Jensen's inequality,
$\Exp [ h(x) ] \ge h (\Exp [x])$,
so we have
%
\begin{align}
\Exp_{\valvec \sim F}
\left[
\left(
\frac{1}%
{1 + \sum_{j = 1}^{\numbidders - 1} \mathbbm{1}_{\val[j] \ge \val(\hat{q})}}
\right)^{1/d}
\right]
&\ge
\left(
\frac{1}%
{1 + \Exp_{\valvec \sim F}
\left[
\sum_{j = 1}^{\numbidders - 1} \mathbbm{1}_{\val[j] \ge \val(\hat{q})}
\right]}
\right)^{1/d}
\\
&=
\left(
\frac{1}%
{1 + (\numbidders - 1) \hat{q}}
\right)^{1/d}
,\end{align}
%
and
\begin{align}
APX
&\ge
\sum_{i = 1}^{\numbidders}
\left(
\frac{1}%
{1 + (\numbidders - 1) \hat{q}}
\right)^{1/d}
\val(\hat{q})^{1/d}
\hat{q}
\\
&=
\numbidders
\left(
\frac{\val(\hat{q})}%
{1 + (\numbidders - 1) \hat{q}}
\right)^{1/d}
\hat{q}
.\end{align}
%
\end{proof}


With Lemma~\ref{lem:reserveQuantileApx}
and Theorem~\ref{thm:pseudoSurplusUbMhr},
we can now describe the performance of the 
mechanism when the reserve is the median $\kappa$
(i.e., $\hat{q} = \frac{1}{2}$).

\begin{theorem}
\label{thm:apxRatioMedianDgeTwo}
The approximation ratio of the mechanism with median reserve price $\kappa$
in a symmetric environment, when, $\forall i \in \bidders$, 
$\costfun[i] = \payment[i]^d$, 
where $d \ge 2$
with MHR distributions, is:
\begin{align}
\label{eq:postedPriceMedianRatioDgeTwo}
\frac{APX}{OPT}
&\ge
\frac{1}{2} 
\left(\frac{2 \numbidders}{e (\numbidders + 1)}\right)^{1/d}
.\end{align}
\end{theorem}

\begin{proof}
%
Lemma~\ref{lem:reserveQuantileApx} tells us that when $\hat{q} = \frac{1}{2}$,
\begin{align}
APX
&\ge
\numbidders
\left(
\frac{\kappa}%
{1 + (\numbidders - 1) / 2}
\right)^{1/d}
\frac{1}{2}
\\
&=
\frac{\numbidders}{2}
\left(
\frac{2 \kappa}%
{\numbidders + 1}
\right)^{1/d}
,\end{align}
%
and by Theorem~\ref{thm:pseudoSurplusUbMhr},
we have:
\begin{align}
\frac{APX}{OPT}
&\ge
\frac{\numbidders}{2}
\left(
\frac{2 \kappa}%
{\numbidders + 1}
\right)^{1/d}
\frac{1}{\numbidders^{(d-1)/d} (e \kappa)^{1/d}}
\\
&=
\frac{1}{2}
\left(
\frac{2 \numbidders}%
{e(\numbidders + 1)}
\right)^{1/d}
.\end{align}
%
\end{proof}

Equation~\eqref{eq:postedPriceMedianRatioDgeTwo}
tells us that for large number of bidders,
the approximation ratio is $\frac{1}{2} \left(\frac{2}{e} \right)^{1/d}$.
As $d \ge 2$, this is at least $0.42$.
Further, as $d$ tends towards infinity, the approximation ratio approaches $\frac{1}{2}$.
Thus, using distribution knowledge improves performance by a factor of $4$
over the prior-free mechanism.

We now observe how the performance of the mechanism changes by using 
the monopoly reserve price $\eta$ instead of median reserve price $\kappa$ 
with the following theorem.
The proof is given in the appendix.
%
\begin{theorem}
\label{thm:apxRatioMonopReserveDgeTwo}
The approximation ratio of the mechanism with monopoly reserve price $\eta$
in a symmetric environment, when, $\forall i \in \bidders$, 
$\costfun[i] = \payment[i]^d$, 
where $d \ge 2$
with MHR distributions, is:
\begin{align}
\label{eq:apxRatioMonopReserveDgeTwo}
\frac{APX}{OPT}
&\ge
\left(
\frac{1}{e}
\frac{\numbidders (1 - F(\eta))^{d-1}}{1 + (\numbidders - 1) (1 - F(\eta))}
\right)^{1/d}
.\end{align}
\end{theorem}










We explore how well mechanisms with reserve prices do empirically using randomly generated
MHR distributions in Section~\ref{sec:Experiments}.

